Fast Inverter Control by Learning the OPF Mapping using Sensitivity-Informed Gaussian Processes

Fast inverter control is a desideratum towards the smoother integration of renewables. Adjusting inverter injection setpoints for distributed energy resources can be an effective grid control mechanism. However, finding such setpoints optimally requires solving an optimal power flow (OPF), which can be computationally taxing in real time. This work proposes learning the mapping from grid conditions to OPF minimizers using Gaussian processes (GPs). This GP-OPF model predicts inverter setpoints when presented with a new instance of grid conditions. Training enjoys closed-form expressions, and GP-OPF predictions come with confidence intervals. To improve upon data efficiency, we uniquely incorporate the sensitivities (partial derivatives) of the OPF mapping into GP-OPF. This expedites the process of generating a training dataset as fewer OPF instances need to be solved to attain the same accuracy. To further reduce computational efficiency, we approximate the kernel function of GP-OPF leveraging the concept of random features, which is neatly extended to sensitivity data. We perform sensitivity analysis for the second-order cone program (SOCP) relaxation of the OPF, whose sensitivities can be computed by merely solving a system of linear equations. Extensive numerical tests using real-world data on the IEEE 13- and 123-bus benchmark feeders corroborate the merits of GP-OPF.

==> latexmkrc.tex <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> old-unused-text.tex <==

% 	\clearpage
% Possible material (open issues in italic):
% \begin{itemize}
% \item Introduction on GPs and how they can be used for differential equations and dynamical systems.
%  \item Power systems dynamics (basic linearized model) + turbine model
% \item Eigenmode decomposition based on homogeneity assumption if we use Model A (see below).
% \item Model A: Model applies on eigenmodes. Each eigenmode is modeled as an independent GP with a Gaussian kernel with its own parameters (alpha,beta). This model brings in spatiotemporal coupling by design. It does not satisfy the Kronecker model. Parameters can be learned through MoM, but in its constrained LS version. Tests work well for this setup.
% \item We need to justify why eigenmodes are modeled as independent.
% \item Model B applies on nodal signals. Each signal is modeled across time using a Gaussian kernel with some parameters (alpha,beta). Signals are spatially coupled through some spatial kernel.
% \item If Model B is confined to have the same temporal kernel across buses, the model adheres to the Kronecker model. In this case, Model B can coincide with Model A if the temporal kernels of Model A are identical across eigenstates. Then, the spatial kernel becomes naturally the inverse Laplacian $\bL$. In this case, we also get a Kronecker model, which has computational advantages (matrix inversion) Unfortunately, Model B does not seem to be working well -- perhaps due to the fact that many parameters are fixed and so there is not much flexibility. 
% \item \emph{Different applications: It is of interest to include power injections in the observed data as well -- especially from generators that are easier to collect as Dr. Zhu suggested. She also suggested adding line power flows, which can be critical too.}
% \item \emph{Tests with actual power systems dynamics: non-homogeneous, non-linear etc.}
% \item \emph{Random features: This could be useful for an online implementation. I'm not sure if it could be useful to help inverting matrices to improve scalability even in the static case.}
% \item \emph{Another option for splitting would be over batch/offline versus online/real-time implementation with some type of RAKER. This would be very pertinent.}
% \item \emph{Low-rank modeling coupled with kernels: We decided to abort this direction, since it is well explored in learning and we are getting closer to low-rank PMU papers.}
% \item \emph{Possible conference/journal split: If a Kronecker model works well, then we can put that on the conference, along with ML estimation. Then, we keep MoM, approximate modeling, equivalences of models, and turbine models for journal. If the latter is worse, we can switch roles so that conference is always the incomplete/worse version of the work, since it comes earlier.}
% \item \emph{Kernel learning in some way (Lanckriet, multi-kernel learning or cross-validation): we aborted this idea too, since it will give us a lot of trouble and again is well studied.}
% \cmb{\emph{We will use their approaches to find which spatial kernel would work the best for ourselves.}}\cmb{ I implemented 15 different spatial kernels and used the alignment criteria introduced in Lanckriet's paper. None of them had a high alignment with the sample covariance matrix.} 
% \item \emph{The direction of learning dynamics and problem parameters at the same time was aborted too. I think it will be too messy.}	    
% 	\end{itemize}
%\begin{remark}\label{re:sys}
%			As mentioned earlier, the inertia and damping coefficients are assumed to be known here. However, GP estimation scheme is able to handle estimating the required parameters using some information on the input signals which can be obtained from the SCADA measurements. To this end, the measurement vector $\tbz$ should be altered to $\tbz=[\tbtheta^\top \tbomega^\top \tbp^\top]^\top$. The frequency estimation follows the procedure described in~\eqref{eq:m_zz}-~\eqref{eq:sigma} with the new $\tbz$ with the difference that the SISO parameters $\gamma$ and $\{\lambda_i\}_{i=1}^N$ can be assumed to be additional parameters prior parameters to be estimated~\cite{raissi17}. In this case, the method of moments is not applicable for parameter selection. Instead, one can resort to the traditional method of maximizing the marginal likelihood. maximum likelihood estimation of parameters favors an embedded regularizer which prohibits overfitting and suffers from nonconvexity which may result in local minima solutions. 
%			The SCADA measurements of $\tbp$ are sampled less frequently compared to the PMU data which can be captured by the covariance kernel function~\eqref{eq:kernel}. It is important to notice that not all input data have to be measured in order to find the system parameters. Due to the fact that the prior parameters are in eigenspace, the minimum needed measurements depend on the participation factors of the eigenmodes. 
%\end{remark}

%Similar to decomposing the swing equations, we adopt several assumptions for transforming the primary control system into multiple SISO systems. Along with the homogeneity assumption of $\bD=\gamma \bM$, we assume the eigenvector matrix $\bV$ diagonalizes matrices $\bT$, $\bR$, and $\bM$ such that


	%Frequencies across the buses in a power system are linear combinations of the eigenspace variables. We modeled the eigenspace variables as GPs to facilitate the Bayesian estimation discussed in Section~\eqref{eq:x2}. 
	%Frequencies being a linear combination of the eigenspace variables, can also be expressed as GPs. Modeling all the signals in a power system as GPs leverages the possibility of applying Bayesian-based estimation techniques for finding the non-metered signals. In Section~\ref{sec:formula}, the goal was to infer the behavior of signals in a SISO LTI system. The focus here is to study the behavior of MIMO LTI systems in~\eqref{eq:swing} and~\eqref{eq:turbine2} using the GP framework. The challenge of inferring the outputs of a MIMO system can be narrowed down to capturing the spatial and temporal coupling among the system states. 
	
%	\color{blue}
	%Eigenspace variables are the basis components of the power system states. By modeling the eigenspace variables as Gaussian processes, temporal covariance of each eigenstate can be defined as $\mathbb{E}[\by_i \by_i^\top]=\alpha_i \bK_i$. Abusing the independence of eigenmodes statistical independence can be assumed among eigenspace variables, which implies $\mathbb{E}[\by_i \by_j^\top]=\bzero, \ \forall i\neq j$. The angles and frequencies across all the buses are a combination of the eigenmodes characterized by the eigenvectors of $\bL_M$. The spatial coupling of the system states can be captured by these eigenvectors. It is worth noting that the spatial coupling between two buses does not necessarily depend on the physical distance between them. The spatial coupling across a system measures how similar buses respond to a disturbance. Each eigenmode responds differently to a power disturbance. On the other hand, different eigenmodes have different influences on each state variable, characterized by the eigenvectors of $\bL_M$ according to~\eqref{eq:trans}. Hence, the correlation of two buses can be categorized by the similarity of the eigenvectors mapping them to the eigenstates. Based on this intuition, the spatiotemporal covariance of the frequencies and angles across buses is formulated next.
	%\color{black}
	%Once the temporal covariances of the eigenstates are defined, the linear mapping~\eqref{eq:trans} automatically captures the spatial coupling of the states. 
	
		%\begin{equation}\label{eq:vec}
	%\tbtheta:=\mathrm{vec}(\hbTheta^\top), \quad \tbomega:=\mathrm{vec}(\hbOmega^\top).
	%\end{equation}
	%Various types of PMUs are installed in a power system, providing angle and frequency measurements with different accuracies. Assuming independence between the measurements, using both angle and frequency data offers better results. To this end, we introduce new variables $\hbZ \in \mathbb{R}^{2M \times T}$ and $\tbz \in \mathbb{R}^{2MT}$, where
	%\begin{equation}\label{eq:z}
	%\hbZ:=[\hbTheta^\top ~ \hbOmega^\top]^\top, \quad \tbz := [\tbtheta^\top ~ \tbomega^\top]^\top. 
	%\end{equation}
	
		%The concatenation of $\tbz$ and $\bomega_n$ is the GP
	%\begin{equation}
	%\begin{bmatrix}
	%\tbz\\
	%\bomega_n
	%\end{bmatrix} \sim \mcN\left( \bzero , \begin{bmatrix}
	%\mathbb{E}[\tbz \tbz^\top] & \mathbb{E}[\tbz \bomega_n^\top]\\
	%\mathbb{E}[\bomega_n \tbz^\top] &\mathbb{E}[\bomega_n \bomega_n^\top]
	%\end{bmatrix}\right).
	%\end{equation}
	
		%\begin{equation}
	%\label{eq:c_zz}
	%\mathbb{E}[\tbz \tbz^\top]=\begin{bmatrix}
	%\mathbb{E}[\tbtheta \tbtheta^\top] && \mathbb{E}[\tbtheta \tbomega^\top]\\
	%\mathbb{E}[\tbomega \tbtheta^\top] && \mathbb{E}[\tbomega \tbomega^\top]
	%\end{bmatrix}.
	%\end{equation}
	
	%\begin{proposition}\label{prop:turbine}
	%    If the eigenvectors corresponding to $\bL$ can diagonalize matrices $\bM,~\bD,~\bR^{-1}, \bT$, the power system modeled by~\eqref{eq:turbine2} can be transformed into multiple SISO systems using the following transformations
	%    \begin{equation}\label{eq:trans_turbine}
	%       \btheta=\bU \bz, \quad \bp=\bU \bu 
	%   \end{equation}
	%   where $\bU$ is based on the eigenvalue decomposition $\bL = \bU \bGamma \bU^\top, \ \bGamma:=\{\gamma_1,\dots,\gamma_N\}$.
	%\end{proposition}
	%\emph{Proof:} Substitute~\eqref{eq:trans_turbine} into~\eqref{eq:turbine1} and multiplying both sides with $\bU^\top$.
	
	
	
%%%%% STATISTICAL INFERENCE SECTION by Mana
% 	Consider PMU measurements are available for buses $\mcM:=\{1,\dots,M\}$ at times $\mcT$. The noisy measurements of the angles, frequencies, and power mismatches are collected in $\hbTheta, \hbOmega, \hbP \in \mathbb{R}^{M\times T}$. Given measurements PMU measurements, the goal is to estimate $\omega_n(t); \ n \notin \mcM$. One of the advantages of the GP toolbox is that the non-metered buses can be estimated for $t \notin \mcT$. The GP framework described in Section~\ref{sec:GP} will be employed for inferring the states of the non-metered buses. 
	
% Finding $\omega_n(t)$ using the Bayesian method requires the covariance matrices $\mathbb{E}[\theta_n(t) \theta_{n'}(t')]$, $\mathbb{E}[\theta_n(t) \omega_{n'}(t')]$, $\mathbb{E}[\theta_n(t)p_{n'}(t')]$, etc. To construct the spatiotemporal covariances the measurements are expressed as 
% 	\begin{equation}
% 	    \tbp=\mathrm{vec}(\hbP), \ \tbtheta=\mathrm{vec}(\hbTheta), \ \tbomega=\mathrm{vec}(\hbOmega)
% 	\end{equation}
% 	Furthermore, all measurements will be collected in $\tbz:=[\tbtheta^\top,\tbomega^\top,\tbp^\top]^\top$. Using the Bayesian method, the frequency $\omega_n=\omega_n(t)$ can be estimated by the conditional expectation
% 	%\begin{equation}\label{eq:m_ff}
% 	%	\mathbb{E}[\bomega_n|\hbomega]=\mathbb{E}[\bomega_n \hbomega^\top] \left( \mathbb{E}[\hbomega \hbomega^\top] \right)^{-1} \hbomega, \quad n=M+1,\dots,N.
% 	%\end{equation}
% 	\begin{equation}\label{eq:m_zz}
% 	\mathbb{E}[\omega_n|\tbz]=\mathbb{E}[\omega_n \tbz^\top] \left( \mathbb{E}[\tbz \tbz^\top] \right)^{-1} \tbz.
% 	\end{equation}
% 	 Similar to the SISO system, the uncertainty of the inference of $\omega_n$ can be measured using the diagonal entries of
% 	\begin{equation}\label{eq:v_zz}
% 	\mathbb{E}[\omega_n\omega_n^\top|\tbz]=\mathbb{E}[\omega_n\omega_n^\top]- \mathbb{E}[\omega_n \tbz^\top] \left( \mathbb{E}[\tbz\tbz^\top] \right)^{-1} \mathbb{E}[\tbz \omega_n ^\top].
% 	\end{equation}
% 	First, we focus on formulating the covariance across angles, which implies finding the correlation of angles between two time instances $t,t'$ and across buses $n,n'$. In the model 
% 	\begin{equation*}
% 	    \hbtheta(t)=\bM^{-1/2}\bV \by(t)
% 	\end{equation*}
% 	the eigenspace variable is the only function of time. Hence the temporal covariance is captured by the covariances of the eigenspace variables. We model the eigenspace variables independent from each other
% 	\begin{align*}
% 	    \mathbb{E}[y_i(t)y_j(t')]=\begin{cases}
% 	    \alpha_i k_i(t,t'), \quad &~t_i=t_j\\
% 	    0, \quad &~t_i \neq t_j.
% 	    \end{cases}
% 	\end{align*}
% 	Independence of the eigenspace variables reduces the number of parameters in the model; instead of $N^2$ number of $\alpha_{ij}$s, there are only $N$ number of $\alpha_i$s in the model. 

%     To see how the dynamics are spatially coupled consider the phase angle measurements
% 	\begin{equation}\label{eq:trans2}
% 	\hbTheta := \bS \bM^{-1/2} \bV \bY +\bE
% 	\end{equation} 
% 	where $\bS\in \mathbb{R}^{M \times N}$ selects the $M$ entries corresponding to the metered buses. The eigenspace variables and noise are collected in matrices $\bY\in \mathbb{E}^{N\times T}$ and $\bE \in \mathbb{E}^{M\times T}$. Vectorizing $\hbTheta$ and using the Kronecker product properties gives
% 	\begin{equation}
% 	\tbtheta=\left(\bS \bM^{-1/2} \bV \otimes \bI_T \right) \mathrm{vec}(\bY^\top)+ \mathrm{vec}(\bE^\top).
% 	\end{equation}
% 	By defining $\tby:=\mathrm{vec}(\bY^\top)$ and $\bSigma:=\mathbb{E}[ \mathrm{vec}(\bE^\top) \mathrm{vec}(\bE^\top)^\top ]$ the covariance matrix $\mathbb{E}[\tbtheta \tbtheta^\top]$ can be formulated as
% 	\begin{equation}\label{eq:c_tt}
% 	\mathbb{E}[\tbtheta \tbtheta^\top]=(\bS \bM^{-1/2} \bV \otimes \bI_T) \mathbb{E}[\tby \tby^\top] (\bV^\top \bM^{-1/2} \bS^\top\otimes \bI_T)+\bSigma.
% 	\end{equation}
% 	The spatiotemporal covariance of $\hbTheta$ is defined by~\eqref{eq:c_tt}. 
	
% 	\begin{proposition}\label{pro:spatiotemporal}
% 		Due to the independence of the eigenmodes from each other, the temporal covariance between the eigenspace variables is a block-diagonal matrix
% 		\begin{equation}\label{eq:c_ytyt}
% 		\mathbb{E}[\tby \tby^\top]=\bdiag(\alpha_1\bK_1,\dots,\alpha_N\bK_N).
% 		\end{equation}
% 		Each $\alpha_i\bK_i$ is the temporal covariance of the eigenspace variable $i$. The temporal covariances of the system states are linear mappings of the temporal covariances of the eigenspace variables due to~\eqref{eq:trans}. The mapping between the covariances of the system states and the eigenstate variables automatically picks up the spatial covariance of state variables across buses and forms~\eqref{eq:c_tt}.
% 	\end{proposition}
% 	%\emph{\textbf{Proposition:} The covariance matrix~\eqref{eq:c_tt} is the spatio-temporal covariance between the metered angles and frequencies across the system. 
% 		%The covariance matrix $\mathbb{E}[\tby \tby^\top]$ is the temporal covariance between the eigenspace variables. Due to the independence of eigenmodes from each other, $\mathbb{E}[\tby \tby^\top]$ is a block-diagonal matrix
% 		%\begin{equation}
% 		%\mathbb{E}[\tby %\tby^\top]=\bdiag(\alpha_1\bK_1,\dots,\alpha_N\bK_N).
% 		%\end{equation}
% 		%The mapping between the state and eigenstate variables automatically picks up the spatial covariance of state variables across buses.}
% 	Other covariance matrices can be modeled in a similar fashion. For example $\mathbb{E}[\tbomega\tbomega^\top]$ is similar to~\eqref{eq:c_tt} with the difference that $\mathbb{E}[\dot{\tby}\dot{\tby}^\top]$ would be replaced $\mathbb{E}[\tby \tby^\top]$. The covariance matrix between the derivative of the eigenspace variables is
% 	\begin{equation}
% 	    \mathbb{E}[\tby \tby^\top]=\bdiag(\alpha_1\dot{\bK}_1,\dots,\alpha_N\dot{\bK}_N).
% 	\end{equation}
% 	where $\dot{\bK}_i$ is defined in~\eqref{eq:kdot}. 



%Monitoring power system oscillations is crucial for maintaining stability. Undamped oscillations jeopardize the stability and the synchronization of the system, stress the machinery, and restrain the power flow on the transmission lines~\cite{pai_stability}. Detecting the sources of oscillations helps to prevent large-scale outages. Finding the undamped modes of oscillation and localizing the sources of disturbances in a system require information about the dynamic signals in the power system. The integration of phasor measurement units(PMUs) has provided frequently sampled measurements of the dynamic signals across the grid. However, many of the buses in the system are not metered by PMUs. Moreover, due to communication issues and PMU malfunctions, the available PMU measurements are sparse. Estimation of the non-metered and missing PMU data is an important step in analyzing the dynamic signals in a power system.











% \begin{table}
% 	\renewcommand{\arraystretch}{1.2}
% 	\caption{Average RPE [\%] and standard deviation (std) [$\times 10^{-3}$]\\
% 	and execution times [s] of prediction the OPF solutions}
% 	\label{tbl:est} \centering
% 	\begin{tabular}{|l|r|r|r|r|r|}
% 		\hline\hline
% 	    \multirow{2}{*}{$T= 35$, $D=800$} &   \multicolumn{2}{c|}{\textbf{$\bq^g$}} & \multicolumn{2}{c|}{\textbf{$\bp^g$}} & \multirow{2}{*}{\textbf{Time}}\\
% 	   \cline{2-5}
% 	    &  RPE & std & RPE & std &   \\
% 		\hline\hline \textbf{GPR}& $4.2$ & $0.7$ & $4.56$ & $0.59$ & $0.013$\\
% 		\hline	\textbf{SI-GPR}& $3.62$ & $1.1$ & $3.17$ & $0.34$ & $0.83$\\
% 		\hline	\textbf{RF-GPR}& $4.32$ &$0.68$& $4.68$  & $0.57$  & $0.02$ \\
% 		\hline	\textbf{SI-RF-GPR}&  $3.92$ &$0.52$& $3.97$  & $0.41$  & $0.14$ \\
% 		\hline\hline
% 	\end{tabular}
% \end{table}

% \begin{table}
% 	\renewcommand{\arraystretch}{1.2}
% 	\caption{Average RPE [\%] and standard deviation (std) [$\times 10^{-3}$]\\
% 	and execution times [s] of prediction the OPF solutions}
% 	\label{tbl:est2} \centering
% 	\begin{tabular}{|l|r|r|r|r|r|}
% 		\hline\hline
% 	    \multirow{2}{*}{$T = 57$, $D=800$} &   \multicolumn{2}{c|}{\textbf{$\bq^g$}} & \multicolumn{2}{c|}{\textbf{$\bp^g$}} & \multirow{2}{*}{\textbf{Time}}\\
% 	   \cline{2-5}
% 	    &  RPE & std & RPE & std &   \\
% 		\hline\hline \textbf{GPR}& $3.28$ & $0.48$ & $4.32$ & $0.31$ & $0.016$\\
% 		\hline	\textbf{SI-GPR}& $2.7 $ & $ 0.4$ & $2.62$ & $0.24 $ & $2.63$\\
% 		\hline	\textbf{RF-GPR}& $ 3.39$ &$0.46 $& $4.33$  & $0.3$  & $0.023 $ \\
% 		\hline	\textbf{SI-RF-GPR}&  $3 $ &$ 0.36$& $3.31$  & $0.22 $  & $0.11$ \\
% 		\hline\hline
% 	\end{tabular}
% \end{table}

% \begin{table}
% 	\renewcommand{\arraystretch}{1.2}
% 	\caption{Average time for parameter estimation, training, and prediction. }
% 	\label{tbl:time} \centering
% 	\begin{tabular}{|l|r|r|r|r|r|r|}
% 		\hline\hline
% 	    \multirow{2}{*}{\textbf{}} &   \multicolumn{3}{c|}{\textbf{Training}} & \multicolumn{2}{c|}{\textbf{Prediction}}&  \\
% 	   \cline{2-7}
% 	    &  MLE & MMSE & std& MMSE & std & overall \\
% 		\hline\hline \textbf{GPR}& $0.66$ & $0.01$ &$--$& $0.002$ & $0.001$& $0.67$\\
% 		\hline	\textbf{SI-GPR}& $1.59$ & $69$ &$--$&  $0.02$ &  $0.06$& $70.67$\\
% 		\hline	\textbf{RF-GPR}& $0.66$ & $0.14$ & $0.05$ &$0.0005$& $0.0013$& $0.85$\\
% 		\hline	\textbf{SI-RF-GPR}& $1.59$ & $0.52$ & $0.03$ & $0.0008$& $0.001$& $2.14$\\
% % 		\hline	\textbf{OPF}& $--$ & $--$ & $--$ & $--$ & $--$ & $3.34$\\
% 		\hline\hline
% 	\end{tabular}
% \end{table}
